A divergence preserving cut finite element method for Darcy flow

We study cut finite element discretizations of a Darcy interface problem based on the mixed finite element pairs $\textbf{RT}_k\times Q_k$, $k\geq 0$. Here $Q_k$ is the space of discontinuous polynomial functions of degree less or equal to $k$ and $\textbf{RT}$ is the Raviart-Thomas space. We show that the standard ghost penalty stabilization, often added in the weak forms of cut finite element methods for stability and control of the condition number of the linear system matrix, destroys the divergence-free property of the considered element pairs. Therefore, we propose new stabilization terms for the pressure and show that we recover the optimal approximation of the divergence without losing control of the condition number of the linear system matrix. We prove that the method with the new stabilization term has pointwise divergence-free approximations of solenoidal velocity fields. We derive a priori error estimates for the proposed unfitted finite element discretization based on $\textbf{RT}_k\times Q_k$, $k\geq 0$. In addition, by decomposing the mesh into macro-elements and applying ghost penalty terms only on interior edges of macro-elements, stabilization is applied very restrictively and only where needed. Numerical experiments with element pairs $\textbf{RT}_0\times Q_0$, $\textbf{RT}_1\times Q_1$, and $\textbf{BDM}_1\times Q_0$ (where $\textbf{BDM}$ is the Brezzi-Douglas-Marini space) indicate that we have 1) optimal rates of convergence of the approximate velocity and pressure; 2) well-posed linear systems where the condition number of the system matrix scales as it does for fitted finite element discretizations; 3) optimal rates of convergence of the approximate divergence with pointwise divergence-free approximations of solenoidal velocity fields. All three properties hold independently of how the interface is positioned relative to the computational mesh.

==> Errorestimatesold.tex <==
\section{Analysis of the Method}\label{sec:analysis}
Proofs for well-posedness of the unstabilized unfitted method \eqref{eq:unstabdarcy} exist only for the lowest order pair $\RT_0\times Q_0$ \cite{DanSco12}, to the best of our knowledge. Despite this, using a direct solver, the unstabilized method succeeds in approximating the exact solution in all our numerical experiments with optimal convergence order. However, the resulting linear systems could be severely ill-conditioned in particular in case of high order elements, we illustrate this in the next Section. The analysis of Method 1 would to a large extent follow from the work in~\cite{puppi2021cut}. However, this method does not preserve the divergence-free property of the $\bfH^{\dive}$-conforming elements. We propose to use Method 2. Thus, we only analyze Method 2 and throughout this section we assume $\bfV_k=\RT_k$ and hence $\hat{k}=k$.

We start by defining the following mesh dependent norms: 
\begin{align}
\| q \|^2_h &:= 
	\sum_{i\in\{1,2\}}\sum_{T\in\mcT_{h,i}} \| q_{i} \|^2_T = \| q \|^2_{\Omdh}, \\
    \tn \bfv \tn^2_\Af &:= \Af(\bfv,\bfv) \nonumber \\
    &= \|\permi^{1/2}\bfv\|^2_{\Omega_1\cup\Omega_2} +\|\permig^{1/2}\{\bfv\cdot\pmb{n}\}\|^2_{\interf} + \xi \|\permig^{1/2}\jump{\bfv\cdot\pmb{n}}\|^2_{\interf} + s_{\bfu}(\bfv,\bfv),  \label{eq:anorm}\\
	\tn \bfv \tn^2_h &:= \tn \bfv \tn_\Af^2 + \| \dive \bfv\|_{\Omdh}^2=\tn \bfv \tn_\Af^2 + \| \dive \bfv\|_{h}^2.\label{eq:vhnorm}
% |r|_{\ell} &:= \sum_{i\in\{1,2\}}\sum_{T\in\mcT_{h,i}} |r|^2_{\ell,T}.
\end{align}
%Here $|r|_{\ell,T}$ is the standard seminorm of order $\ell$ over $T,$ and $r$ can be either scalar or vector valued.



Next we state some properties of standard interpolants for our spaces that we will use.  

Let $\projpi:L^2(\Omdhi)\to \Qki$ be the orthogonal projection on $\Qki$ and $\interpvi : \bfH^{\dive}(\Omdhi)\cap \prod_{T\in\mcT_{h,i}} \bfH^r(T) \to \Vki$, ($r\geq 1$), be the global interpolation operator associated to $\Vki$, \review{see e.g. \cite[(2.5.10)-(2.5.27)]{BofBreFor13} and \cite[Chapter 3]{Gatica14}.} The following commuting diagram holds \review{(see \cite[diagram (2.5.27)]{BofBreFor13} or \cite[Lemma 3.7]{Gatica14})}:
\begin{equation}\label{eq:diagram}
	\begin{tikzcd}
		\bfH^{\dive}(\Omega_{\mcT_{h,i}})\cap \prod_{T\in\mcT_{h,i}} \bfH^{r}(T) \arrow{r}{\dive} \arrow[swap]{d}{\pi_{h,i}^k} & L^2(\Omega_{\mcT_{h,i}}) \arrow{d}{\projpi} \\%
		\Vki \arrow{r}{\dive} & \Qki
	\end{tikzcd}
\end{equation}

%The global Raviart-Thomas interpolation operator $\interpvi$ is continuous in the following sense, 
%\begin{equation} \label{eq:stabilityintp}
%\|\interpvi\bfv\|_{\bfH^{\dive}(\Omdhi)} \lesssim \|\bfv\|_{\bfH^1(\Omdhi)}, \quad  \forall \bfv \in \bfH^1(\Omdhi).
%\end{equation}
%See Lemma 4.4 in \cite{Gatica14}.

The following local interpolation error estimates hold:
\begin{lemma}\textbf{(Local interpolation error estimates)}\label{lem:loc_interp}
	Fix $T\in\mcT_{h}$. Let $\bfu\in\bfH^{k+1}(T)$, $\dive\bfu\in H^{k+1}(T)$, then for $0\leq m\leq \ell+1$ and $0\leq \ell \leq k$,
	\begin{align*}
	| \bfu-\interpvi \bfu |_{m,T} &
        \lesssim h^{\ell+1-m}|\bfu|_{\ell+1,T}, \\
	| \dive\bfu-\dive\interpvi \bfu |_{m,T} &
        \lesssim h^{\ell+1-m}|\dive\bfu|_{\ell+1,T}.
	\end{align*} 
\end{lemma} 
For a proof see Lemma 3.16 and 3.17 of \cite{Gatica14}.

We will also make use of the following elementwise trace inequalities. For $T\in \mesh$  we have the trace inequalities
\begin{equation} \label{eq:tracestand}
\| v \|^2_{L^2(\partial T)} \lesssim h^{-1} \| v \|_{L^2(T)}^2 + h \| \nabla v \|^2_{L^2(T)} \qquad v\in H^1(T), 
\end{equation} 
\begin{equation} \label{eq:trace}
\| v \|^2_{L^2(T\cap \Gamma)} \lesssim h^{-1} \| v \|_{L^2(T)}^2 + h \| \nabla v \|^2_{L^2(T)} \qquad v\in H^1(T),
\end{equation} 
where the first inequality is a standard trace inequality, see, e.g.~\cite{BreSco}, and the second inequality is proven in \cite{HaHaLa04} and the constant 
is independent of how $\Gamma$ intersects $T$ and of $h$. 


\subsection{Stability} \label{sec:stability}
Before we state and prove an inf-sup result for $\Bf$ we state two Lemmas we will need.    
\begin{lemma}\textbf{(The Poincaré inequality)}\label{lem:Poincare}
	Let $D$ be a bounded Lipschitz domain in $\RR^d$
        with $\emptyset\neq S\subset \partial D$
        and let $\bfv\in\bfH_{0,S}^1(D)$. Then, 
	\begin{align*}
		\|\bfv\|_{D} \leq C_P \|\nabla\bfv\|_{D},
	\end{align*} 
	where $C_P=2$diam$(D)$.
\end{lemma}
See Theorem 7.91 in \cite{Salsa2016}.

%\begin{lemma}\label{lem:divergence_Poincare}
%  Let $D$ be a polygonal domain in $\RR^d$ or have a smooth boundary $\partial D$. %$\emptyset\neq S\subset\partial D$ a subset of its boundary.
%        Then for any $q\in L^2(D)$ there exists a $\bfv \in \bfH_{0,S}^1(D)$ with $\emptyset\neq S\subset\partial D$, satisfying 
%	\[\dive\bfv = q,\ \|\bfv\|_{\bfH^1(D)}\leq C \|q\|_{D}, \]
%        where $C$ is a positive constant independent of q. If $q$ satisfies $\int_D q=0$ then $\bfv \in \bfH_{0}^1(D)$.  
%\end{lemma} 
\begin{lemma}\label{lem:divergence_Poincare}
  \review{Let $D$ be a bounded convex polygonal domain in $\RR^d$ or a bounded open subset of $\RR^d$ with a smooth boundary $\partial D$.
    %$\emptyset\neq S\subset\partial D$ a subset of its boundary.
        Then there exist a positive constant C such that for all $q\in L^2(D)$ there is a $\bfv \in \bfH^1(D)$ satisfying 
	\[\dive\bfv = q,\ \|\bfv\|_{\bfH^1(D)}\leq C \|q\|_{D}. \]
        If $q$ satisfies $\int_D q=0$ then $\bfv \in \bfH_{0}^1(D)$.}  
\end{lemma} 
See Lemma 11.2.3 in \cite{BreSco}. %Lemma 4.7 in \cite{DanSco12} and 
\review{We will use this lemma in the inf-sup proof and apply it in the domain %$\Omeps=\Omega_i \cup U_{\varepsilon}(\Gamma) \subset \RR^d$, where
  $U_{\varepsilon}(\Gamma)$,  an open tubular $\varepsilon$-neighborhood of $\Gamma$ with $0<\varepsilon\leq \varepsilon_0$.} %We do this construction to get an inf-sup constant independent of the mesh size parameter $h$.
We assume $\Gamma$ is a smooth closed simply connected surface. Let $U_{\varepsilonz}(\Gamma)$ be an open tubular neighborhood of $\Gamma$ with thickness $\varepsilonz>0$ such that for each $\bfx \in U_{\varepsilonz}(\Gamma)$ there is a uniquely determined $p(\bfx) \in \Gamma$. Note that $\varepsilonz$ is a constant that depends on the curvature of the surface $\Gamma$. For a surface with high curvature the constant $\varepsilonz$ is small. We also assume that $h$ is sufficiently small so that $\bigcup_{T \in \mathcal{G}_h } T \subset U_{\varepsilon}(\Gamma)$ and $\Omdhi \subset \Omeps$ for $\varepsilon=ch\leq \varepsilonz$.
\begin{prop}(\textbf{The inf-sup condition}) \label{prop:infsup}
For every $q_h\in \Qk$ there exists a constant $\beta>0$ independent of the mesh size function $h$ such that 
\begin{align}
\sup_{\bfv_h\in \Vk} \frac{\Bf(\bfv_h,q_h)}{\tn \bfv_h \tn_h} \geq \beta \|q_h\|_h. 
\label{eq:inf sup proposition} 
\end{align}
\end{prop}

\begin{proof}
\review{Fix $q_{h}=(q_{h,1},q_{h,2}) \in \Qk$. Let}
\begin{equation}
  \hat{q}=
  \left \{
  \begin{tabular}{ll}
  $q_{h,1}$ & \textrm{in $\Omega_1$,} \\
  $q_{h,2}$ & \textrm{in $\Omega_2$.}
  \end{tabular}
  \right.
\end{equation}
Then, let $\bfv_p \in \bfH^{1}(\Omega)$ %with $S\subset\partial \Omega$
%($S=\partial\Omega \setminus \partial\Omega_p$)
be the function from Lemma \ref{lem:divergence_Poincare} satisfying 
\begin{align} 
&\dive \bfv_p =-\hat{q} \quad \textrm{ in $\Omega$,}   \label{eq:vp} 
\\
&\|\bfv_p\|_{\bfH^1(\Omega)} \lesssim \|\hat{q}\|_{\Omega}. %=\|q_{h,i}\|_{\Omdhi}.
\label{eq: vpnorm}
\end{align} 
Note that in case $\boundp=\emptyset$ we have $\int_{\Omega_1 \cup \Omega_2} q_h=0$.  This is consistent with the result we get from Lemma \ref{lem:divergence_Poincare} with $\bfv_p \in \bfH^{1}_{0}(\Omega)$  since 
  \[0=\int_{\partial\Omega}\bfv_p\cdot\bfn=\int_{\Omega}\dive\bfv_p = -\int_{\Omega} \hat{q}=0.\]  
  
Further for each $i=1,2$ extend $q_{h,i}$ defined in $\Omdhi$ by zero to $\Omepsz$ and denote this extension by $q_{h,i}^e$. Applying Lemma \ref{lem:divergence_Poincare} with $D=\intfneig$ and $q_{h,i}^e \in L^2(\intfneig)$ we know that there exist a $\bfv_i^e \in \bfH^{1}_{0,S_i}(\intfneig)$ with $\emptyset\neq S_i \subset\partial \intfneig$ ($S_i$ belongs to the part of the boundary that is outside $\Omdhi$) such that 
\begin{align}
&\dive \bfv_i^e =-q_{h,i}^e \quad \textrm{ in $\intfneig$,}   \label{eq:vi} 
\\ 
&\|\bfv_i^e\|_{\bfH^1(\intfneig)} \lesssim \|q_{h,i}^e\|_{\intfneig}. \label{eq:vinorm}
\end{align} 
  Let $\bfv_{h}=(\bfv_{h,1}, \bfv_{h,2}) \in \Vk$ be the Raviart-Thomas interpolant of $\bfv_p$ on the uncut elements in $\Omega_{h,i}$ and of $\bfv_i^e$ on the cut elements:   
\begin{equation}\label{eq:defvhi}
  \bfv_{h,i} = \interpvi \bfv_i
  \quad \textrm{with }
 %\begin{equation}
 \bfv_i =  \left \{
  \begin{tabular}{ll}
   $\bfv_p$  & \textrm{for $T \in \mcT_{h,i} \setminus \mathcal{G}_h$,} \\
   $\bfv_i^e$ & \textrm{for $T \in \mathcal{G}_h$.}
  \end{tabular}
  \right.
%\end{equation} 
  %\left \{
  %\begin{tabular}{ll}
  % $\interpvi \bfv_p$  & \textrm{in $\uncutdom$,} \\
  %   $\interpvi \bfv_i^e$ & \textrm{in $\cutdom$}
  % \end{tabular}
  %\right.  
\end{equation}
Note that $\bfv_i \in \bfH^{\dive}(\Omega_{\mcT_{h,i}})\cap \prod_{T\in\mcT_{h,i}} \bfH^{1}(T)$ with $\dive \bfv_i = -q_{h,i}$ in $\Omdhi$ and we have from the commuting diagram the identity (see \cite[Theorem 3.2 and Lemma 3.7]{Gatica14}):
\begin{align}
\dive\bfv_{h,i}= -q_{h,i} \quad \textrm{in $\Omdhi$.}
\label{eq: commuting property}
\end{align}
Thus, for $q_{h}=(q_{h,1},q_{h,2})$ and $\bfv_{h}=(\bfv_{h,1},\bfv_{h,2})$ we have
\begin{align*}
	\Bf(\bfv_{h},q_{h}) &= -(\dive \bfv_{h},q_{h})_{\Omega_1\cup\Omega_2} - s_b(\bfv_{h},q_{h})\\
	&= \|q_{h} \|_{\Omega_1\cup\Omega_2}^2 + s_b(q_h, q_h)
        \gtrsim \| q_{h} \|^2_h,
\end{align*}
with the last inequality being an application of Lemma \ref{lem:sp_ineq}. We are done if we can show that $\tn \bfv_h \tn_h \lesssim \| q_h\|_h$.

Recall the definition of the norm $\tn \bfv_{h} \tn_h^2$,
\begin{align*}
	\tn \bfv_{h} \tn_h^2 &= \underbrace{\|\permi^{1/2}\bfv_h\|^2_{\Omega_1\cup\Omega_2}+ \|\dive\bfv_h\|^2_{\Omdh} }_{\mathbf{I}}
	+
	\underbrace{s_{\bfu}(\bfv_h,\bfv_h)}_{\mathbf{II}}
	+
	\underbrace{ \|\permig^{1/2}\{\bfv_h\cdot\pmb{n}\}\|^2_{\interf} + \xi \|\permig^{1/2}\jump{\bfv_h\cdot\pmb{n}}\|^2_{\interf}}_{\mathbf{III}}.
\end{align*}

\textbf{Term I}. Recall our choice of $\bfv_{h,i}$ (see equation \eqref{eq:defvhi}). First note that using local interpolation estimates, Lemma \ref{lem:loc_interp} with $l=m=0$, we have 
\begin{align}\label{eq:intponv}
	\|\bfv_{h,i}\|^2_{T} &\lesssim \|\bfv_i-\bfv_{h,i}\|^2_{T}  + \|\bfv_i\|^2_{T} \lesssim h^2\|\nabla\bfv_i\|^2_{T} + \|\bfv_i\|^2_{T} \lesssim \|\bfv_i\|^2_{\bfH^1(T)}. 
\end{align}
Next using that $\bigcup_{T \in \mathcal{G}_h } T \subset \intfneig$ together with equations \eqref{eq: vpnorm} and \eqref{eq:vinorm} and that $q_{h,i}^e=0$ outside $\Omdhi$  we obtain
\begin{align}
\sum_{i=1}^2 \sum_{T\in\mcT_{h,i}} \|\bfv_i\|_{\bfH^1(T)} 
&
%\lesssim \sum_{i=1}^2\left(\sum_{T\in\mcT_{h,i} \setminus \mathcal{G}_h} 
%\|\bfv_p\|_{H^1(\uncutdom)}+\sum_{T\in \mathcal{G}_h} \|\bfv_i\|_{H^1(\cutdom)} \right)
\lesssim
\|\bfv_p\|_{\bfH^1(\Omega)}+\sum_{i=1}^2\|\bfv_i^e\|_{\bfH^1( \intfneig)}
%\nonumber \\
\lesssim \sum_{i=1}^2 \left(\|q_{h,i}\|_{\Omega_i}+\|q_{h,i}^e\|_{\intfneig} \right) \lesssim
\sum_{i=1}^2\|q_{h,i}\|_{\Omdhi}.
\label{eq:estimatvinq}
\end{align}
Applying \eqref{eq: commuting property}-\eqref{eq:estimatvinq} we get 
\begin{align}
\|\permi^{1/2}\bfv_h\|^2_{\Omega_1\cup\Omega_2}+ \|\dive\bfv_h\|^2_{\Omdh}  \lesssim \sum_{i=1}^2\sum_{T\in\mcT_{h,i}} \left(\|\bfv_{h,i}\|_{T}^2+\|\dive \bfv_{h,i}\|_{T}^2 \right) \lesssim  \|q_h\|^2_h.
\end{align}

\textbf{Term II}. Using a standard elementwise trace inequality followed by the standard inverse inequality to remove $j-1$ derivatives,  see e.g. \cite{BreSco}, we obtain 
\begin{align}\label{eq:stabbound}
& s_{\bfu}(\bfv_{h},\bfv_{h})=
\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} \tau_{u} \left( h \|\jump{\pmb{v}_{h,i}}\|^2_{F}  + \sum_{j=1}^{\kp+1} h^{2j + 1} \|\jump{D^j_{\bfn_F} \pmb{v}_{h,i}}\|^2_{F} \right)  \nonumber \\
& \quad  \lesssim  
\sum_{i=1}^2\sum_{T\in\mcT_{h,i}} \left( \| \bfv_{h,i}\|_{T}^2 + \sum_{j=1}^{\kp+1} h^{2j} h^{2-2j} \| \bfv_{h,i} \|_{\bfH^1(T)}^2 \right).
\end{align}
Local interpolation estimates, see Lemma \ref{lem:loc_interp}, yield
\begin{align}\label{eq:H1bound}
	\|\bfv_{h,i}\|^2_{\bfH^1(T)} &\lesssim \|\bfv_i-\bfv_{h,i}\|_{\bfH^1(T)}^2 + \|\bfv_i\|_{\bfH^1(T)}^2 \lesssim \|\bfv_i\|^2_{\bfH^1(T)}.
\end{align}
Applying this estimate together with \eqref{eq:estimatvinq} we get
\begin{align}
& s_{\bfu}(\bfv_{h},\bfv_{h}) \lesssim  
%\sum_{i=1}^2\sum_{T\in\mcT_{h,i}} \left( \| \bfv_{h,i}\|_{T}^2 +
% \sum_{j=1}^{\kp+1} h^{2} \| \bfv_{h,i} \|_{\bfH^1(T)}^2 \right)
%  \lesssim 
 \sum_{i=1}^2 \sum_{T\in\mcT_{h,i}} \| \bfv_i\|_{\bfH^1(T)}^2 %\\
  \lesssim \|q_h\|^2_h.
\end{align}


\textbf{Term III}.  
We handle the interface terms by applying an elementwise trace inequality followed by the standard inverse inequality, the estimate in \eqref{eq:intponv}, using that $\cup_{T\in\mcGh} T \subset U_\varepsilon(\Gamma)$ and on this tubular neighborhood we apply the Poincaré inequality, Lemma \ref{lem:Poincare}. We finally use that $\varepsilon=ch$. Thus,   
\begin{align} 
  \|\bfv_{h,i}\cdot \pmb{n}\|^2_{\interf} &=\sum_{T\in\mcGh} \|\bfv_{h,i}\cdot \pmb{n}\|^2_{\interf\cap T}
  \lesssim h^{-1} \sum_{T\in\mcGh}\|\bfv_{h,i}\|^2_{T} %\\ \nonumber
	%&
        \lesssim h^{-1} \sum_{T\in\mcGh}(h^2\|\nabla\bfv^e_i\|^2_{T}+\|\bfv^e_i\|^2_{T}) \\ \nonumber
       	&\lesssim h\|\nabla\bfv_i^e\|^2_{U_\varepsilon(\Gamma)}+ h^{-1}\|\bfv_i^e\|^2_{U_\varepsilon(\Gamma)} \\ \nonumber
	&\lesssim \max(h,h^{-1}\varepsilon^2) \|\bfv_i^e\|^2_{\bfH^1(U_\varepsilon(\Gamma))} \lesssim \|q_{h,i}\|^2_{\Omdhi},
\end{align}
with the last inequality being due to \eqref{eq:vinorm} and since $q_{h,i}^e=0$ outside $\Omdhi$.

After splitting up averages and jump terms and applying the above estimate we get,
\begin{align}\label{eq:termI-IV}
	\|\permig^{1/2}\{\bfv_h\cdot\pmb{n}\}\|^2_{\interf} + \xi \|\jump{\permig^{1/2}\bfv_h\cdot\pmb{n}}\|^2_{\interf}
	 \lesssim \sum_{i=1}^2\|q_{h,i}\|^2_{\Omdhi} = \|q_h\|^2_h.
\end{align}
 
Combining the estimates for \textbf{Term I-III} yields the desired inequality,  
\begin{align*}
	\tn \bfv_{h} \tn_h^2 &\lesssim  \| q_{h} \|_h^2. 
\end{align*}    
\end{proof}


\subsection{Interpolation error estimates}\label{sec:interpol}
To define the interpolant we need extensions of functions in $\Omega_i$ to $\Omdhi$.
We need extension operators
\begin{equation}
	\bfE_i: \Hdivinto(\Omega_i)\to \Hdivinto(\RR^d),\
        \hat{E}_i: H^{\intorp}(\Omega_i)\to H^{\intorp}(\RR^d), 
\end{equation}
with $\intorp\geq 1$, that for $\bfv_i\in\Hdivinto(\Omega_i)$ and $q_i\in H^{\intorp}(\Omega_i)$ satisfy
\begin{align}
\|\bfE_i\bfv_i\|_{\Hdivinto(\RR^d)} &\lesssim \|\bfv_i\|_{\Hdivinto(\Omega_i)},
\quad (\bfE_i \bfv_i)|_{\Omega_i}=\bfv_i \text{ a.e.},
\label{eq:sobo_velbound}\\
\|\hat{E}_i  q_i\|_{H^{\intorp}(\RR^d)} &\lesssim \|q_i\|_{H^{\intorp}(\Omega_i)}, \quad
 (\hat{E}_i q_i)|_{\Omega_i}=q_i \text{ a.e.}, \label{eq:sobo_presbound}\\
\dive\circ \bfE_i &= \hat{E}_i \circ \dive.\label{eq:commdiagE}
\end{align}
The Sobolev-Stein extension operators satisfy these properties, see \cite[(3.16) and Corollary 4.1]{Hiptmair2012Universal}. 
%, see also \cite{puppi2021cut}.
We can then define

\begin{equation}
	\bfE: \bigoplus_{i=1}^2 \Hdivinto(\Omega_i) \ni (\bfv_1, \bfv_2) \to (\bfE_1 \bfv_1, \bfE_2 \bfv_2) \in \bigoplus_{i=1}^2 \Hdivinto(\RR^d),
\end{equation}

\begin{equation}
	\hat{E}: \bigoplus_{i=1}^2 H^{\intorp}(\Omega_i) \ni (q_1, q_2) \to (\hat{E}_1  q_1, \hat{E}_2  q_2) \in \bigoplus_{i=1}^2 H^{\intorp}(\RR^d),
\end{equation}
and finally the following interpolation and projection operators

\begin{equation}\label{eq:defintpv}
\interpv : \bigoplus_{i=1}^2 \Hdivinto (\Omega_i) \ni (\bfv_1, \bfv_2) \to \left(\pi_{h,1}^k \left(\bfE_1\bfv_1|_{\Omega_{\mcT_{h,1}}}\right), \pi_{h,2}^k \left(\bfE_2\bfv_2|_{\Omega_{\mcT_{h,2}}}\right) \right) \in \Vk, 
\end{equation}

\begin{equation}\label{eq:defintpp}
\interpp : \bigoplus_{i=1}^2 H^{\intorp}(\Omega_i) \ni (q_1, q_2) \to \left(\projpii{1} \left(\hat{E}_1q_1|_{\Omega_{\mcT_{h,1}}}\right), \projpii{2} \left(\hat{E}_2 q_2|_{\Omega_{\mcT_{h,2}}}\right) \right)\in \Qk. 
\end{equation}
%Note that for the Raviart-Thomas element pair $\hat{k}=k$. 
\begin{lemma}\textbf{(Interpolation/projection estimates)}\label{lem:interp}
	Let $\bfu\in \bigoplus_{i=1}^2 \Hdivinto(\Omega_i)$ and $p\in \bigoplus_{i=1}^2 H^{\intorp}(\Omega_i)$, then
        \begin{align}
	 \tn \bfE \bfu-\interpv \bfu \tn_h &\lesssim h^{k+1/2}\sum_{i=1}^2\left(\|\bfu_i\|_{\bfH^{k+1}(\Omega_i)} + \|\dive\bfu_i\|_{H^{k+1}(\Omega_i)} \right),\label{eq:interpresu} \\
        \| \hat{E}p-\interpp p \|_h &\lesssim h^{k+1}\sum_{i=1}^2 \|p_i\|_{H^{k+1}(\Omega_i)}.\label{eq:interpresp}
        \end{align}
\end{lemma}
\begin{proof}
Let $\interr= \bfE \bfu-\interpv \bfu$. Recall that 
	\begin{align*}
		\tn \interr \tn_h^2 &= 
		\|\permi^{1/2}\interr \|^2_{\Omega_1\cup\Omega_2}  + \|\dive\interr \|^2_{\Omdh} +
		s_{\bfu}(\interr, \interr)	+
		\|\permig^{1/2}\{\interr \cdot\pmb{n}\}\|^2_{\interf} + \xi \|\permig^{1/2}\jump{\interr \cdot\pmb{n}}\|^2_{\interf}.
	\end{align*}
Using local interpolation estimates from Lemma \ref{lem:loc_interp} and the properties of the extension operators, \eqref{eq:sobo_velbound}-\eqref{eq:commdiagE}, we have
\begin{align}
\|\permi^{1/2}\interr_i\|^2_{\Omega_i}& \lesssim \sum_{T\in \mcTh}\|\permi^{1/2}\interr_i\|^2_{T} \lesssim h^{2(k+1)} \sum_{T\in \mcTh} |\bfE_i \bfu_i |^2_{k+1,T} \lesssim h^{2(k+1)} \| \bfu_i \|^2_{\bfH^{k+1}(\Omega_i)},\label{eq:interpboundI} \\
	\|\dive \interr_i \|^2_{\Omdhi} &= \sum_{T\in \mcTh} \|\dive \interr_i \|^2_{T} \lesssim h^{2(k+1)} \sum_{T\in \mcTh} |\dive \bfE_i\bfu_i |^2_{k+1,T} 
		=h^{2(k+1)} \sum_{T\in \mcTh} |\hat{E}_i \dive \bfu_i|_{k+1,T}^2  \nonumber \\
                &\lesssim h^{2(k+1)} \| \dive\bfu_i \|^2_{H^{k+1}(\Omega_i)}. \label{eq:interpboundI_2}
\end{align}

Next we look at the stabilisation term. We use an elementwise trace inequality, followed by local interpolation estimates ($\|D^j\interr_i\|_{T}\lesssim h^{k+1-j}|\bfE_i\bfu_i|_{k+1,T}$ from Lemma \ref{lem:loc_interp}), and the stability of the extension operator to get
\begin{align}
	s_{\bfu}(\interr, \interr)&=\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} \tau_{u} \left(\sum_{j=0}^{k+1} h^{2j + 1} \|\jump{D^j_{\bfn_F} \interr_i}\|^2_{F} \right) \lesssim \sum_{i=1}^2 \sum_{T \in \mcGh} \left( 
	\sum_{j=0}^{k+1} h^{2j+1}\left(h^{-1}\|D^j \interr_i\|_{T}^2+h\|D^{j+1} \interr_i\|_{T}^2 \right) \right) \nonumber \\
	&\lesssim h^{2(k+1)}\sum_{i=1}^2 \sum_{T\in \mcTh} | \bfE_i \bfu_i |^2_{k+1,T} \lesssim h^{2(k+1)}\sum_{i=1}^2 \| \bfu_i \|^2_{\bfH^{k+1}(\Omega_i)}. \label{eq:interpboundII}
\end{align}
For the interface terms we again use an elementwise trace inequality, followed by local interpolation estimates, and the stability of the extension operator. We get
 
\begin{align}
	\|\interr_i \cdot \pmb{n}\|^2_{\interf} &%\lesssim
	 %\sum_{T\in\mcGh} \|\interr_i\cdot \pmb{n}\|^2_{T} 
	\lesssim \sum_{T\in\mcGh} \left(h^{-1} \|\interr_i\|^2_{T}
+h \|D \interr_i\|^2_{T} \right)
\nonumber \\
	&\lesssim h^{2k+1}\sum_{T\in\mcTh}|\bfE_i\bfu_i|^2_{k+1,T} 
	\lesssim h^{2k+1}\|\bfu_i\|_{\bfH^{k+1}(\Omega_i)}^2.
\end{align} 
Summing all terms together we get the desired estimate \eqref{eq:interpresu}. Since $\|\cdot \|_h$ is just the broken $L^2$-norm on the active meshes, the estimate \eqref{eq:interpresp} follows from standard estimates and using the stability of the extension operator $\hat{E}_i$, see \eqref{eq:sobo_presbound}. 
\end{proof}

\begin{remark}\textbf{The interpolation estimate}
	The interface terms are the only terms which contribute to the $h^{k+1/2}$ scaling of the interpolation estimate. For all other terms we get $h^{k+1}$. 
	We note that it is not possible to take the interpolation estimates of Lemma \ref{lem:loc_interp} beyond $|\bfu|_{k+1,T}$ in the hopes of picking up an extra power of $h$. For example for $k=0$ one can construct a linear function $\bfv$ on an element $T$ so that $\bfv \in \bfQ_1(T)\setminus\RT_0(T)$. If the local interpolation estimates of Lemma \ref{lem:loc_interp} could go to $|\cdot|_{2,T},$ then
	\begin{align}
		|\bfv-\interpv \bfv|_{0,T}\lesssim h^2|\bfv|_{2,T}=0,
	\end{align}
	which is a contradiction due to the construction of $\bfv$ and that $\interpv \bfv$ is a function in $\RT_0(T)$.
\end{remark} 

\subsection{Consistency and continuity}\label{sec:consistency}
Before we are ready to show a priori error estimates we need to show a result on consistency of Method 2 and that the bilinear forms $\Af$ and $\Bf$ are continuous.

\begin{lemma}(\textbf{Consistency})\label{lem:consist}
Let $\bfu \in \bfV \cap \bigoplus_{i=1}^2 \Hdivinto(\Omega_i)$ and $p \in \bigoplus_{i=1}^2 H^{k+1}(\Omega_i)$ be the solution to \eqref{eq:weakdarcy}-\eqref{eq:weakdarcy2}. Let $(\bfu_h,p_h)\in\Vk\times\Qk$ be the solution to \eqref{eq:discretedarcy2}-\eqref{eq:discretedarcy2b}. Then,
\begin{align}
	\Af(\bfu_h-\bfE \bfu,\pmb{v}_h) + \Bf(\bfv_h, p_h-\hat{E} p) &=-s_{\bfu}(\bfE \bfu,\bfv_h),
        \quad \forall \bfv_h \in \Vk,\label{eq:consisteq1}\\
	\Bf(\bfu_h-\bfE \bfu,q_h) &= 0, \quad \forall q_h \in \Qk,
\end{align}
with
\begin{equation}\label{eq:suforEu}
  s_{\bfu}(\bfE \bfu,\bfv_h)= \sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}}
\tau_{\bfu} h^{2k+3}  (\jump{D^{k+1}_{\bfn_F} \bfE_i \bfu_i }, \jump{D^{k+1}_{\bfn_F} \bfv_{h,i}})_{F}.
\end{equation}

\end{lemma}
 
\begin{proof} 
  Note that since $\hat{E_i}p_i \in H^{k+1}(\RR^d)$ and $\bfE_i \bfu_i \in \Hdivinto(\RR^d)$ we have $\jump{D^{j} \hat{E_i}p_i}=0$, $\jump{D^j (\dive (\bfE_i \bfu_i)}=0$, and $\jump{D^{j}_{\bfn_F} (\bfE_i \bfu_i)^l}=0$   for $0\leq j \leq k$, ($l=1, \cdots, d$). Hence $s_b(\bfv_h,\hat{E}p)=s_b(\bfE \bfu, q_h)=0$ and consequently $\Bf(\bfE \bfu, q_h)=b(\bfu, q_h)$ and $\Bf(\bfv_h, \hat{E} p)=b(\bfv_h, p)$. Furthermore, equation \eqref{eq:suforEu} holds. Following the derivation of the weak form \eqref{eq:weakdarcy}-\eqref{eq:weakdarcy2}, we get 
\begin{align}
  \Af(\bfu_h-\bfE \bfu,\bfv_h) + \Bf(\bfv_h, p_h-\hat{E} p) &= \FF (\pmb{v}_h)-\left(a(\bfu, \bfv_h)+\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}}
  \tau_{\bfu} h^{2k+3} ([D^{k+1}_{\bfn_F} \bfE_i \bfu_i ], [D^{k+1}_{\bfn_F} \bfv_{h,i}])_{F}  + b(\bfv_h, p) \right), \nonumber \\
  	\Bf(\bfu_h-\bfE \bfu,q_h) &= 0, \nonumber
\end{align}
and the result follows. 
\end{proof}

\begin{lemma}\textbf{(Continuity)}\label{lem:continuity}
The bilinear forms $\Af$ and $\Bf$ are continuous
	\begin{align}
		\Af(\bfv,\bfw) &\lesssim \tn \bfv \tn_h \tn \bfw \tn_h, \quad \forall \bfv, \bfw \in \left(\bigoplus_{i=1}^2\Hdivinto(\Omdhi)+\Vk \right),  \\ 
		\Bf(\bfv,q) &\lesssim \tn \bfv \tn_h\|q\|_h, \quad \forall \bfv \in \left(\bigoplus_{i=1}^2\Hdivinto(\Omdhi)+\Vk \right), \ q \in \bigoplus_{i=1}^2\left(H^{k+1}(\Omdhi) + \Qki \right).
                %\textcolor{purple}{\| \dive \bfv\|_h \|q\|_h } \lesssim
	\end{align}
\end{lemma}
\begin{proof}
	Applying Cauchy-Schwartz we see that $\Af(\bfv,\bfw) \lesssim \Af(\bfv,\bfv)^{1/2}\Af(\bfw,\bfw)^{1/2}$ whereby the first inequality follows. To show that $\Bf$ is continous we again apply Cauchy-Schwartz,
	\begin{align}\label{eq:contB}
		\Bf(\bfv,q) &= -(\dive\bfv,q)_{\Omega_1\cup\Omega_2}-s_b(\bfv,q) \lesssim \| \dive\bfv \|_{\Omega_1\cup\Omega_2} \|q\|_{\Omega_1\cup\Omega_2} + |s_b(\bfv,q)| \nonumber \\
		&\lesssim \| \dive\bfv \|_{\Omega_1\cup\Omega_2} \|q\|_{\Omega_1\cup\Omega_2}  + s_p(\dive\bfv,\dive\bfv)^{1/2}s_p(q,q)^{1/2} \nonumber \\ 
		&\lesssim\| \dive\bfv \|_{h}\|q\|_{h} \lesssim \tn\bfv\tn_h\|q\|_h.
	\end{align}
        Note that for the stabilization term we have used that for $q_h \in \Qk$ an elementwise trace inequality followed by the standard inverse inequality to remove $j$ derivatives yields
\begin{align}\label{eq:stabbound}
& s_{p}(q_{h},q_{h})=
\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} \tau_p \left( h \|\jump{q_{h,i}}\|^2_{F}  + \sum_{j=1}^{k} h^{2j + 1} \|\jump{D^j q_{h,i}}\|^2_{F} \right)  \nonumber \\
& \quad  \lesssim  
\sum_{i=1}^2 \left( \| q_{h,i}\|_{\Omdhi}^2 + \sum_{T\in\mcT_{h,i}}\sum_{j=1}^{k} h^{2j} h^{-2j} \| q_{h,i} \|_{T}^2 \right)\lesssim \| q_{h} \|_{h}^2.
\end{align}
Furthermore, for $q_i \in H^{k+1}(\Omdhi)$ and $\dive \bfv_i \in  H^{k+1}(\Omdhi)$, we have $\jump{D^j q_{i}}=0$ and $\jump{D^j (\dive \bfv_{i})}=0$ for $0\leq j \leq k$. Thereof, $s_p(q,q)^{1/2} \lesssim \|q\|_h$ and $s_p(\dive\bfv,\dive\bfv)^{1/2} \lesssim \| \dive\bfv \|_{h}$ in equation \eqref{eq:contB}.    

\end{proof}


\subsection{A priori error estimates}\label{sec:apriori}
When the exact divergence is in the pressure space, $\dive\bfE\bfu\in\Qk$, the saddle-point structure of our problem allows us to mimic the a priori proof for standard FEM, see \cite[Theorem 2.6]{Gatica14}. However, for the general case 
we have to couple the pressure error with the velocity error. We introduce for $\bfu_h,\bfv_h\in\Vk,p_h,q_h\in\Qk,$
\begin{align}
	\Cf((\bfu_h,p_h),(\bfv_h,q_h)) &:= \Af(\bfu_h,\bfv_h) +\Bf(\bfv_h,p_h)+
	\Bf(\bfu_h,q_h) = \FF (\pmb{v}_h) + \GG(q_h), \\
	\tn (\bfv_h,q_h) \tn^2_h &:= \tn \bfv_h\tn^2_h + \|q_h\|^2_h,
\end{align}
next we prove a stability result, and finally we show optimal a priori error estimates. 
\begin{lemma}\label{lem:big_infsup}
	For any $(\bfrho_h,\sigma_h)\in \Vk\times\Qk$ there exists $(\bfw_h,r_h)\in \Vk\times\Qk$ such that 
	\begin{align}
          \Cf((\bfrho_h,\sigma_h),(\bfw_h,r_h))\gtrsim \tn (\bfrho_h,\sigma_h) \tn_h^2, \quad
          \tn (\bfw_h,r_h) \tn_h \lesssim \tn (\bfrho_h,\sigma_h) \tn_h.
	\end{align}
\end{lemma}  
\begin{proof}
	Let $-\bfv_h\in\Vk$ be the element attaining the inf-sup condition in Proposition \ref{prop:infsup}, that is $\Bf(-\bfv_h,\sigma_h)\gtrsim \|\sigma_h\|^2_h$, and $\tn\bfv_h\tn_h \lesssim \|\sigma_h\|_h$. Using also continuity of the bilinear form $\Af$ and Young's inequality we have
	\begin{align}
		\Cf((\bfrho_h,\sigma_h),(-\bfv_h,0)) &= -\Af(\bfrho_h,\bfv_h)+\Bf(-\bfv_h,\sigma_h) \nonumber \\
		&\gtrsim -\tn\bfrho_h\tn_h\tn\bfv_h\tn_h + \|\sigma_h\|^2_h \gtrsim -\tn\bfrho_h\tn_h\|\sigma_h\|_h + \|\sigma_h\|^2_h \nonumber \\
		&\gtrsim -\epsilon^{-1}\tn\bfrho_h\tn^2_h + (1-\epsilon)\|\sigma_h\|^2_h.
	\end{align}
Using Lemma \ref{lem:sp_ineq} we have $\Bf(\bfrho_h, -\dive\bfrho_h)=\|\dive \bfrho_h\|^2_{\Omega_1 \cup \Omega_2}+ s_p(\dive \bfrho_h, \dive \bfrho_h) \gtrsim \|\dive \bfrho_h\|^2_{h}$ and hence, 
	\begin{align}
		\Cf((\bfrho_h,\sigma_h),(\bfrho_h,-\dive\bfrho_h-\sigma_h)) &= \Af(\bfrho_h,\bfrho_h)+\Bf(\bfrho_h,\sigma_h)+\Bf(\bfrho_h, -\dive\bfrho_h-\sigma_h)\nonumber \\
		&\gtrsim \tn\bfrho_h\tn^2_{\Af} +  \|\dive \bfrho_h\|^2_{h}= \tn\bfrho_h\tn^2_{h}.
	\end{align}
        Choosing $(\bfw_h,r_h)=(\bfrho_h-\delta\bfv_h,-\dive\bfrho_h-\sigma_h)$ with $\delta>0$ we have
	\begin{align}
		\Cf((\bfrho_h,\sigma_h),(\bfrho_h-\delta\bfv_h,-\dive\bfrho_h-\sigma_h))
		&\gtrsim (1-\delta\epsilon^{-1}) \tn\bfrho_h\tn^2_{h} + \delta(1-\epsilon)\|\sigma_h\|^2_h \gtrsim \tn (\bfrho_h,\sigma_h) \tn^2_h, 
	\end{align}
        to get the last inequality we can for instance choose $\epsilon=1/2$ and $\delta=1/3$. Using that $\| \dive\bfrho_h \|_h \lesssim \tn \bfrho_h \tn_h$ and $\tn \bfv_h \tn_h \lesssim \|\sigma_h\|_h$ we also have that
	\begin{align}
          \tn (\bfw_h,r_h) \tn_h \lesssim \tn \bfrho_h-\delta\bfv_h\tn_h+ \| \dive\bfrho_h+\sigma_h\|_h %\lesssim \tn \bfrho_h \tn_h+\delta \tn \bfv_h \tn_h
          \lesssim \tn (\bfrho_h,\sigma_h) \tn_h.
	\end{align}
\end{proof}

\begin{thm}(\textbf{A priori error estimate})
	Let $\bfu \in \bfV\cap \bigoplus_{i=1}^2 \Hdivinto(\Omega_i)$ and $p \in \bigoplus_{i=1}^2 H^{k+1}(\Omega_i)$ be the solution to \eqref{eq:weakdarcy}-\eqref{eq:weakdarcy2}. Let $(\bfu_h,p_h)\in\Vk\times\Qk$ be the solution to \eqref{eq:discretedarcy2}-\eqref{eq:discretedarcy2b}. Then,
	\begin{align}
		\tn \bfE \bfu-\bfu_h \tn_h
+	\| \hat{E}p-p_h \|_h 
&\lesssim h^{k+1/2}\sum_{i=1}^2\left(\|\bfu_i\|_{\bfH^{k+1}(\Omega_i)} + \|\dive\bfu_i\|_{H^{k+1}(\Omega_i)}+\|p_i\|_{H^{k+1}(\Omega_i)}\right).
\end{align}
\end{thm}
\begin{proof}
Adding and subtracting the interpolant and using the triangle inequality we have,
\begin{align}
\tn \bfE\bfu-\bfu_h \tn_h \leq  \tn \bfE\bfu-\interpv\bfu \tn_h + \tn \bfu_h-\interpv\bfu \tn_h, \\
\|\hat{E}p-p_h\|_h\leq \|\hat{E}p-\interpp p\|_h + \|p_h-\interpp p\|_h.  
\end{align}
We now want to estimate $\tn \bfu_h-\interpv\bfu \tn_h +\|p_h-\interpp p\|_h$ in terms of $\tn \bfE\bfu-\interpv\bfu \tn_h+ \|\hat{E}p-\interpp p\|_h$. Applying Lemma \ref{lem:big_infsup} to $(\bfrho_h, \sigma_h)=(\bfu_h-\interpv\bfu, p_h-\interpp p)$, we have that there exist $(\bfw_h,r_h)\in \Vk\times\Qk$ such that 
\begin{align}\label{eq:stabC}
  \tn (\bfrho_h,\sigma_h) \tn_h^2 \lesssim  \Cf((\bfrho_h,\sigma_h),(\bfw_h,r_h)), \quad 
\tn (\bfw_h,r_h) \tn_h \lesssim \tn (\bfrho_h,\sigma_h) \tn_h.
\end{align}
Consistency (Lemma \ref{lem:consist}) and continuity of the bilinear forms $\Af$ and $\Bf$ (Lemma~\ref{lem:continuity}) together with Cauchy-Schwartz inequality ($s_{\bfu}(\bfE \bfu,\bfw_h)\leq s_{\bfu}(\bfE \bfu,\bfE \bfu)^{1/2} s_{\bfu}(\bfw_h,\bfw_h)^{1/2}$) yield
\begin{align}
		\left|\Cf((\bfrho_h,\sigma_h),(\bfw_h,r_h))  \right|&
		= \left|\Af(\bfu_h-\interpv\bfu,\bfw_h) +\Bf(\bfw_h,p_h-\interpp p)+
		 \Bf(\bfu_h-\interpv \bfu,r_h)\right| \nonumber \\
	  	&= \left|\Af(\bfE\bfu-\interpv\bfu,\bfw_h) +\Bf(\bfw_h,\hat{E}p-\interpp p)+
	 	 \Bf(\bfE\bfu-\interpv \bfu,r_h) 
                 +s_{\bfu}(\bfE \bfu,\bfw_h) \right| \nonumber \\
 		        &\lesssim \left(\tn \bfE\bfu-\interpv\bfu \tn_h+\|\hat{E}p-\interpp p\|_h +  \left(\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} h^{2k+3} \| D^{k+1}_{\bfn_F} \interpv \bfu\|_F^2 \right)^{1/2} \right)\tn (\bfw_h,r_h) \tn_h.
\nonumber 
\end{align} 
In the last step we used that all terms in the stabilization $s_{\bfu}(\bfE \bfu,\bfE \bfu)$ vanish except the last term since $\jump{D^{j}_{\bfn_F} (\bfE_i \bfu_i)^l}=0$ for $0\leq j \leq k$, ($l=1, \cdots, d$) and we added and subtracted the interpolant. Using \eqref{eq:stabC} we end up with the estimate
\begin{align}
  \tn (\bfrho_h,\sigma_h) \tn_h^2  \lesssim  \left(\tn \bfE\bfu-\interpv\bfu \tn_h+\|\hat{E}p-\interpp p\|_h  +\left(\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} h^{2k+3} \| D^{k+1}_{\bfn_F} \interpv \bfu\|_F^2 \right)^{1/2} \right)\tn (\bfrho_h,\sigma_h) \tn_h.
\end{align} 
Using a standard elementwise trace inequality, an inverse estimate, local interpolation estimates (Lemma \ref{lem:loc_interp}), and the stability of the extension operator we have  
\begin{align} \label{eq:consterr}
   \sum_{F \in \mathcal{F}_{h,i}} h^{2k+3} \| D^{k+1}_{\bfn_F} \interpv \bfu\|_F^2 &\lesssim  \sum_{T \in \mathcal{T}_{h,i}} h^{2k+2} \| D^{k+1} \interpv \bfu\|_T^2   \nonumber \\
  &\lesssim
   \sum_{T \in \mathcal{T}_{h,i}} h^{2k+2} \left( \| D^{k+1} (\interpv \bfu-\bfE\bfu)\|_T^2+  \| D^{k+1} \bfE\bfu \|_T^2 \right)  \lesssim
  h^{2k+2} \|\bfu_i\|_{\bfH^{k+1}(\Omega_i)}^2.
  %h^{2k+2} |\bfE\bfu|_{k+1,T}^2. 
\end{align}

Finally, using the interpolation and projection error estimates in Lemma \ref{lem:interp} and \eqref{eq:consterr} we get the result:
\begin{align*}
\tn \bfE\bfu-\bfu_h \tn_h+\|\hat{E}p-p_h\|_h&\lesssim  \tn \bfE\bfu-\interpv\bfu \tn_h +\|\hat{E}p-\interpp p\|_h +\left(\sum_{i=1}^2 \sum_{F \in \mathcal{F}_{h,i}} h^{2k+3} \| D^{k+1}_{\bfn_F} \interpv \bfu\|_F^2 \right)^{1/2}  \\
&\lesssim h^{k+1/2}\sum_{i=1}^2\left(\|\bfu_i\|_{\bfH^{k+1}(\Omega_i)} + \|\dive\bfu_i\|_{H^{k+1}(\Omega_i)}+\|p_i\|_{H^{k+1}(\Omega_i)}\right).
\end{align*}
\end{proof}


